High-energy radiation from collisions of high velocity clouds and the Galactic disk

High-velocity clouds (HVCs) are interstellar clouds of atomic hydrogen that do not partake of the Galactic rotation and have velocities of a several hundred kilometers per second. A considerable number of these clouds are falling down towards the Galactic disk. HVCs form large and massive complexes, so their collisions with the disk must release a great amount of energy into the interstellar medium. The cloud-disk interaction produces two shocks, one propagates through the cloud and the other through the disk; the properties of these shocks depend mainly on the cloud velocity and the disk-cloud density ratio. In this work we study the conditions necessary for these shocks to accelerate particles by diffusive shock acceleration and the produced non-thermal radiation. We analyze particle acceleration in both the cloud and disk shocks. Solving a time-dependent 2-D transport equation for both relativistic electrons and protons we obtain particle distributions and non-thermal spectral energy distributions. In a shocked cloud significant synchrotron radio emission is produced along with soft gamma rays. In the case of acceleration in the shocked disk, the non-thermal radiation is stronger; the gamma rays, of leptonic origin, might be detectable with current instruments. A large number of protons are injected into the Galactic interstellar medium, and locally exceed the cosmic-ray background. We conclude that under adequate conditions the contribution from HVC-disk collisions to the galactic population of relativistic particles and the associated extended non-thermal radiation might be important.

==> figs/figs/caso2/caso2_FP_EN1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(9360.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2340,356){\makebox(0,0){\strut{}8}}%
      \put(3427,356){\makebox(0,0){\strut{}9}}%
      \put(4515,356){\makebox(0,0){\strut{}10}}%
      \put(5603,356){\makebox(0,0){\strut{}11}}%
      \put(6691,356){\makebox(0,0){\strut{}12}}%
      \put(4679,0){\makebox(0,0){\strut{}$\log N$ [erg$^{-1}$ cm$^{-2}$]}}%
      \put(183,1503){\makebox(0,0)[l]{\strut{}$t$  = 0.25  $t_{\rm inj}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \put(4679,4593){\makebox(0,0){\large $E = 10$ Gev}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3303,1503){\makebox(0,0)[l]{\strut{}$t$  = 0.5  $t_{\rm inj}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6423,1503){\makebox(0,0)[l]{\strut{}$t$  = 0.75  $t_{\rm inj}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{caso2_FP_EN1}}%
    \gplfronttext
  \end{picture}%
\endgroup

